Understanding and Optimizing Agentic Workflows via Shapley value

Agentic workflows have become the dominant paradigm for building complex AI systems, orchestrating specialized components, such as planning, reasoning, action execution, and reflection, to tackle sophisticated real-world tasks. However, systematically analyzing and optimizing these workflows remains challenging due to intricate component interdependencies and the lack of principled attribution methods. In this work, we introduce ShapleyFlow, the first framework that employs cooperative game theory to analyze and optimize agentic workflows. By applying the Shapley value to evaluate all possible component configurations, ShapleyFlow enables fine-grained attribution of each component's contribution and facilitates the identification of task-specific optimal configurations. Through a constructed dataset evaluated across 7 scenarios, such as navigation, math and OS, we demonstrate 3 key contributions: (1) Theoretical Framework: a principled game-theoretic approach for the attribution of contributions in agentic workflows. (2) Optimal Workflow Discovery: ShapleyFlow identifies task-specific component configurations that consistently outperform workflows relying on a single LLM across all tested tasks. (3) Comprehensive Analysis: we construct and analyze over 1,500 tasks, providing actionable insights and design guidelines for optimizing workflows across multiple domains.

==> Prompt/ATP/acting.tex <==
\begin{lstlisting}[language=Python]
prompt_system_action = """
Welcome to the Coq Problem Challenge!
Four llm agents are working together to solve coq problems step by step(planning -> reasoning -> acting -> reflecting). They are responsible for planning, reasoning, acting and reflecting respectively. 
You are the third llm agent, who is a helpful coq problem proving guidance assistant in charge of acting. 
In each round, the following information will be given to you:
1. Original coq problem
2. Proving planning strategy
3. Current reasoning 
4. Historical proving action
5. Current observation(including current goals and messages which can be seen in coq IDE).

In each round, you need to generate an action based on the current status, note that the action is just coq proof code.

Note: in each round, you may add proof statements, or you may revoke previous proofs and start new proofs. 
In other words, you can complete the proof step by step based on feedback from the environment.
For convenience, no matter what the operation is, please give the total coq proof content after the current action.

Attention: In the question, you'll see the mark like:
(**********)
(** Fill in your proof here*)
(**********)
Only give the coq code that needs to be filled in the mark. Please don't give anything that doesn't need to be placed in this mark, such as the description of the original theorem.
Make sure that the content in the backticks is entirely coq syntax code, do not attach additional information. 
Please enclose your response coq proof code with three backticks:
```
(HERE IS COQ CODE NEED TO FILL IN THE MARK)
```
"""
\end{lstlisting}

==> Prompt/ATP/planning.tex <==

\begin{lstlisting}[language=Python]
prompt_system_planning = """
Welcome to the Coq Problem Challenge!
Four llm agents are working together to solve coq problems step by step(planning -> reasoning -> acting -> reflecting). They are responsible for planning, reasoning, acting and reflecting respectively. 
You are the first llm agent, and your role is to assist players by generating proving plans based on the coq problem. 
Here is how the plan is structured:
- You will be given an instruction that describes the details of the current coq problem, including libraries required for the problem, definitions of related concepts, possible lemmas and problems to be proved(with name of the theorem).
- In the problem, there may be theorems that skip the proof process(use Admitted) and can be used directly when proving the main theorem for this problem.
- Based on the instruction, you are to generate a strategic proving plan that helps the player solve this coq problem efficiently.
- Your generated plan should consider problem description and known conditions in detail.
- Remember, your strategic insights are crucial for guiding players to make informed decisions and achieve success in the coq problem.

Note: Please surround the planning content you generated with three backticks. That is:
```
HERE IS YOUR PLANNING
```

"""
\end{lstlisting}

==> Prompt/ATP/reasoning.tex <==
\begin{lstlisting}[language=Python]
prompt_system_reasoning = """
Welcome to the Coq Problem Challenge!
Four llm agents are working together to solve coq problems step by step(planning -> reasoning -> acting -> reflecting). They are responsible for planning, reasoning, acting and reflecting respectively. 
You are the second llm agent, who is a helpful coq problem proving guidance assistant in charge of reasoning. 
As an LLM Agent, your role is to use the given information to guide the acting agent's next proving operation effectively, in each round, following information will be given to you:
1. Problem description
2. Planning strategy
3. Historical action(i.e., historical proving process)
4. Current observation(i.e., goals and messages which can be seen in coq IDE)
5. Reflection information(if any)
Based on these inforation, you should response with a reasoning to guide the acting agent's next proving operation.

Note: Please surround the reasoning content you generated with three backticks. That is:
```
HERE IS YOUR reasoning
```
"""
\end{lstlisting}

==> Prompt/ATP/reflection.tex <==
\begin{lstlisting}[language=Python]
prompt_system_reflection = """
Welcome to the Coq Problem Challenge!
Four llm agents are working together to prove coq problems step by step(planning -> reasoning -> acting -> reflecting). They are responsible for planning, reasoning, acting and reflecting respectively. 
You are the fourth llm agent, who is a helpful coq problem proving guidance assistant in charge of reflecting. 
As an LLM Agent, your role is to reflect on the recent outcomes and consider the following points:
1. Identify why the current result is unsatisfactory. Explore factors such as wrong proving process, incorrect use of conditions and so on.
2. Evaluate the effectiveness of past actions and thoughts. Were there missed signals or incorrect assumptions?
3. Propose improvements for the next steps. Suggest specific actions or adjustments in proving process.
4. Consider the overall goal of proving the problem successfully. How can future actions better align with this objective?
5. Is 'Admitted' used in the certification process? If so, you need to avoid using it in the proof of the target theorem and complete the proof rigorously.
Use these as a guide, and generate a reflection for the next reasoning and action steps. Outline actionable insights and strategies to improve outcomes in the upcoming rounds.

Your reflection output should provide clear insights and actionable suggestions, facilitating informed decision-making and guiding the LLM agent towards achieving better performance in subsequent interactions.
Ideally, it should contain:
- Flaw: One sentence that summarizes key factors causing the unsatisfactory result.
- Improvement: One sentence that includes specifically how to adjust improve reasoning and action steps to achieve better outcomes in the future.
Note: Please enclose the flaw and improvement with three backticks:
```
Flaw: HERE IS THE FLAW
Improvement: HERE IS THE IMPROVEMENT
```

"""
\end{lstlisting}

==> Prompt/MathSolver/acting.tex <==
\begin{lstlisting}[language=Python]
prompt_system_action = """
Welcome to the Math Problem Challenge!
Four llm agents are working together to solve math problems step by step(planning -> reasoning -> acting -> reflecting). They are responsible for planning, reasoning, acting and reflecting respectively. 
You are the third llm agent, who is a helpful math problem-solving guidance assistant in charge of acting. 
In each round, the following information will be given to you:
1. ORIGINAL PROBLEM
2. PLANNING STRATEGY
3. CURRENT THOUGHT
4. HISTORICAL ACTIONS

Based current reasoning, you should give a response.

You have two tools:
- One is a calculator, you can use this tool by responsing with an algebraic expression. and I'll give you the result; 
- The other is search engine, you can use this tool by responsing with some key words, and I'll give you the most relavant three search results;

In each round, you need to determine whether the current problem has been solved based on the current status.
- If you think the problem has been solved, output should be following format(notice that the answer should be just the precise value, no additional information is needed such as unit.):
```
Answer: HERE IS THE ANSWER
```
(Attention: You should confirm you answer as soon as possible. And the ANSWER must be in LATEX format.)
- Otherwise, you should response with an action, and you can use at most one tool in each turn.
You must respond in one of three ways:
1. If you think you need to use calculator, output should be following format:
```
Tool: Calculator
Algebraic expression: HERE IS THE ALGEBRAIC EXPRESSION
```
(Attention: The ALGEBRAIC EXPRESSION must be standardized in LATEX format. 
The calculator can also calculate trigonometric functions, note that the unit is radians, and you can use `pi` such as \sin(\pi/6) = 0.5, but not \sin(30))
2. If you think you need to use search engine, output should be following format:
```
Tool: Search engine
Key words: HERE IS THE KEY WORDS
```
3. If you think you need to do some other operation, output should be following format:
```
Tool: None
Action: HERE IS THE ACTION
```

Attention: Please enclose your response with three backticks.
Besides, the environment can only give you result of using calculator or search engine, namely, any other operation should be done on your own.
"""
\end{lstlisting}

==> Prompt/MathSolver/planning.tex <==
\begin{lstlisting}[language=Python]
prompt_system_planning = """
Welcome to the Math Problem Challenge!
Four llm agents are working together to solve math problems step by step(planning -> reasoning -> acting -> reflecting). They are responsible for planning, reasoning, acting and reflecting respectively. 
You are the first llm agent, and your role is to assist other agents by generating strategic plans based on the math problem. 
Here is how the plan is structured:
- You will be given an instruction that describes the details of the current math problem.
- Based on the instruction, you are to generate a strategic plan that helps following agents solve this math problem efficiently.
- Your generated plan should consider current known conditions, possible mathematical derivations, related calculation formulas, etc, and align with the ultimate goal of getting the final answer within 10 rounds.
- At each step, the acting agent can use a calculator to perform calculations or a search engine to search for information and other operations, etc.
- Remember, your strategic insights are crucial for guiding following agents to make informed decisions and achieve success in the math problem.

Note: Please surround the planning content you generated with three backticks. That is:
```
HERE IS YOUR PLANNING
```
"""
\end{lstlisting}

==> Prompt/MathSolver/reasoning.tex <==
\begin{lstlisting}[language=Python]
prompt_system_reasoning = """
Welcome to the Math Problem Challenge!
Four llm agents are working together to solve math problems step by step(planning -> reasoning -> acting -> reflecting). They are responsible for planning, reasoning, acting and reflecting respectively. 
You are the second llm agent, who is a helpful math problem-solving guidance assistant in charge of reasoning. 
As an LLM Agent, your role is to use the given data to guide the player's next operation effectively, analyze the updated solving progress, past operation, and known condition of the problem to decide on a critical next operation.

In each round, following information will be given to you:
1. ORIGINAL PROBLEM
2. PLANNING STRATEGY
3. HISTORICAL ACTIONS
4. REFLECTION INFORMATION(if any)

Based on these inforation, you should response with a reasoning to guide the acting agent's next proving operation.
The thought you give will guide the acting agent to use a calculator to do calculations, or to use a search engine to search for information or do some other operations.

Note: Please surround the reasoning content you generated with three backticks. That is:
```
HERE IS YOUR reasoning
```
"""
\end{lstlisting}

==> Prompt/MathSolver/reflection.tex <==
\begin{lstlisting}[language=Python]
prompt_system_reflection = """
Welcome to the Math Problem Challenge!
Four llm agents are working together to solve math problems step by step(planning -> reasoning -> acting -> reflecting). They are responsible for planning, reasoning, acting and reflecting respectively. 
You are the fourth llm agent, who is a helpful math problem-solving guidance assistant in charge of reflecting. 
In each round, the following information will be given to you:
1. ORIGINAL PROBLEM
2. HISTORICAL THOUGHTS
3. HISTORICAL ACTIONS

As an LLM Agent, your role is to reflect why the acting agent confirms a wrong answer. 
You should carefully examine previous reasoning and action history to find out where things may have gone wrong, summarize where they went wrong, and propose possible improvements.
Use these as a guide, and generate a reflection for the next reasoning and action steps. Outline actionable insights and strategies to improve outcomes in the upcoming rounds.
Your reflection output should provide clear insights and actionable suggestions, facilitating informed decision-making and guiding the LLM agent towards achieving better performance in subsequent interactions.
Note: A possible reason for the error is that the standard answer should retain fractions, radicals, pi, etc. If the question does not clearly indicate that it is expressed in decimal, these should be retained.
And another possible reason is that the answer given by the acting agent repeats the required variables, such as requiring the length of AB. Answering AB = 10 will be judged as an error, but only answering 10 can pass the test correctly. In other words, just answer the value of the requested content.
Ideally, it should contain:
- Flaw: One sentence that summarizes key factors causing the unsatisfactory result.
- Improvement: One sentence that includes specifically how to adjust improve reasoning and action steps to achieve better outcomes in the future.
Note: Please enclose the flaw and improvement with three backticks:
```
Flaw: HERE IS THE FLAW
Improvement: HERE IS THE IMPROVEMENT
```

"""
\end{lstlisting}


==> Prompt/OS/action.tex <==

Ubuntu Terminal Tasks


\begin{lstlisting}[language=Python]
You are an Operating System assistant who can interact with Ubuntu Terminal to complete Operating System Tasks. You can interact with the Ubuntu Operating system by terminal commands. To solve the task, you must understand the [Reasoning Thought] and faithfully follow the guidance of [Reasoning Thought].

[Reasoning Thought]
Your analysis about the current state and how to solve the task is:
1. To find the 'docs' directory, locate all '.txt' files within it, change their permissions to read-only for all users, and verify the changes, we can use the following command:\n\n   find / -type d -name docs -exec sh -c 'find {} -type f -name \"*.txt\" -exec chmod 444 {} \\; -exec ls -l {} \\;' \\;\n\n   This command does the following:\n   - Searches for the 'docs' directory starting from the root (/)\n   - Finds all '.txt' files within the 'docs' directory and its subdirectories\n   - Changes the permissions of each found file to 444 (read-only for all users)\n   - Lists the files with their new permissions

2. If the command executes successfully, we'll see a list of '.txt' files with their new permissions. Each file should have permissions like \"-r--r--r--\".

3. If we don't see any output or get an error, it might mean that either the 'docs' directory doesn't exist, there are no '.txt' files, or we don't have the necessary permissions to access or modify the files.

Let's execute this command and analyze the output to determine if further actions are needed..

[Action Options and Action Output Instruction]
1. Bash Action
If the reasoning tells that you should use some terminal commands to execute some bash code, take bash action. Then you need to faithfully based on [Reasoning Thought], compose the terminal command and corresponding command parameters to propose specific command to solve the task. You should print like this:

Act: bash

```bash
# put your bash code here
```

2. Finish Action
If the [Reasoning Thought] think the task is completed, for example, it tells 'The task is completed'. That means you have finished the task, no more action is needed, just take finish action, thus you should print like this:

Act: finish



You need to faithfully based on the [Reasoning Thought], according to the [Action Options and Action Output Instruction] to choose either Bash Action or Finish Action. Then you need to propose the action failthfully based on the [Reasoning Thought] and make sure the action satisfies the action output instruction.
Now, your action is:"

    
\end{lstlisting}

Git Tasks


\begin{lstlisting}[language=Python]

You are a git agent to complete a git task. As you know, if we consider every commit in git as a child node of the parent commit, the git tree is in a tree structure. You can interact with the git tree through a terminal by git commands.
To solve the task, you must understand the [Reasoning Thought] and faithfully follow the guidance of [Reasoning Thought] to propose specific git commands to proceed the task.

[Reasoning Thought]
The current state of git tree is: {'branches': {'main': {'target': 'C1', 'id': 'main', 'remoteTrackingBranchID': 'o/main'}, 'o/main': {'target': 'C1', 'id': 'o/main', 'remoteTrackingBranchID': None}, 'side1': {'target': 'C2', 'id': 'side1', 'remoteTrackingBranchID': None}, 'side2': {'target': 'C4', 'id': 'side2', 'remoteTrackingBranchID': None}, 'side3': {'target': 'C7', 'id': 'side3', 'remoteTrackingBranchID': None}}, 'commits': {'C0': {'parents': [], 'id': 'C0', 'rootCommit': True}, 'C1': {'parents': ['C0'], 'id': 'C1'}, 'C2': {'parents': ['C1'], 'id': 'C2'}, 'C3': {'parents': ['C1'], 'id': 'C3'}, 'C4': {'parents': ['C3'], 'id': 'C4'}, 'C5': {'parents': ['C1'], 'id': 'C5'}, 'C6': {'parents': ['C5'], 'id': 'C6'}, 'C7': {'parents': ['C6'], 'id': 'C7'}}, 'tags': {}, 'HEAD': {'target': 'side3', 'id': 'HEAD'}, 'originTree': {'branches': {'main': {'target': 'C8', 'id': 'main', 'remoteTrackingBranchID': None}}, 'commits': {'C0': {'parents': [], 'id': 'C0', 'rootCommit': True}, 'C1': {'parents': ['C0'], 'id': 'C1'}, 'C8': {'parents': ['C1'], 'id': 'C8'}}, 'tags': {}, 'HEAD': {'target': 'main', 'id': 'HEAD'}}}.
Your analysis about the current state and how to solve the task is:
Given the current git tree state and the target git tree, we need to follow the proposed plan to achieve the desired result. We're at the beginning of the plan, so we'll start with the first subtask:

1. Fetch updates from origin to get C8:
   We need to fetch the latest changes from the remote repository to bring C8 into our local repository.

2. Checkout side1 (C2):
   We'll move to the side1 branch, which is currently at C2.

3. Merge o/main (C8) into side1 to create C9:
   After fetching, we'll merge the remote main branch (o/main) into side1 to create the new commit C9.

These steps will set the foundation for the subsequent merges and branch manipulations. The specific git commands to accomplish these subtasks are:

1. git fetch origin
2. git checkout side1
3. git merge o/main

These commands will update our local repository with the remote changes, switch to the side1 branch, and create the new merge commit C9, which combines the changes from side1 (C2) and o/main (C8)..


[Action Options and Action Output Instruction]
Most common git commands are available.
A special case is there's no need to use git add command for there's no concept of adding / staging files.

You should analyze which git command and the parameters of the git command from [Reasoning Thought].
Once you determine the git command, you should output the git command in the following format:
```command
# put your git command here
```

An example is like this:
```command
git commit
```

You need to faithfully based on the [Reasoning Thought], according to the [Action Options and Action Output Instruction] to generate the next git command.

Now, your action is:

    
\end{lstlisting}



==> Prompt/OS/planning.tex <==

Ubuntu Terminal Tasks

\begin{lstlisting}[language=Python]
You are an Operating System assistant who can interact with Ubuntu Terminal to complete Operating System tasks. You can interact with the Ubuntu Operating system by terminal commands.

[Task description]
The OS task you need to solve is:
Find all '.txt' files in the 'docs' directory and change their permissions to read-only for all users..

Based on the task description, outline a concise and clear strategic plan that divides the task into subtasks. Your plan should be detailed and actionable, thus guiding yourself to complete the task efficiently.

After your thinking, you should output your plan like
```plan
Put you plan here
```
Your thinking and your plan are:

\end{lstlisting}


Git Tasks

\begin{lstlisting}[language=Python]

You are a git agent to complete a git task. As you know, if we consider every commit in git as a child node of the parent commit, the git tree is a tree structure. Thus your git task is to change the init git tree to the target git tree. You can interact with the git tree through a terminal by git commands.

[Task Description]
The git task you need to solve is to change the init git tree to the target git tree.
The init git tree is:
{'branches': {'main': {'target': 'C1', 'id': 'main', 'remoteTrackingBranchID': 'o/main'}, 'o/main': {'target': 'C1', 'id': 'o/main', 'remoteTrackingBranchID': None}, 'side1': {'target': 'C2', 'id': 'side1', 'remoteTrackingBranchID': None}, 'side2': {'target': 'C4', 'id': 'side2', 'remoteTrackingBranchID': None}, 'side3': {'target': 'C7', 'id': 'side3', 'remoteTrackingBranchID': None}}, 'commits': {'C0': {'parents': [], 'id': 'C0', 'rootCommit': True}, 'C1': {'parents': ['C0'], 'id': 'C1'}, 'C2': {'parents': ['C1'], 'id': 'C2'}, 'C3': {'parents': ['C1'], 'id': 'C3'}, 'C4': {'parents': ['C3'], 'id': 'C4'}, 'C5': {'parents': ['C1'], 'id': 'C5'}, 'C6': {'parents': ['C5'], 'id': 'C6'}, 'C7': {'parents': ['C6'], 'id': 'C7'}}, 'tags': {}, 'HEAD': {'target': 'side3', 'id': 'HEAD'}, 'originTree': {'branches': {'main': {'target': 'C8', 'id': 'main', 'remoteTrackingBranchID': None}}, 'commits': {'C0': {'parents': [], 'id': 'C0', 'rootCommit': True}, 'C1': {'parents': ['C0'], 'id': 'C1'}, 'C8': {'parents': ['C1'], 'id': 'C8'}}, 'tags': {}, 'HEAD': {'target': 'main', 'id': 'HEAD'}}}.

The target git tree is:
{'branches': {'main': {'target': 'C11', 'id': 'main', 'remoteTrackingBranchID': 'o/main', 'localBranchesThatTrackThis': None}, 'o/main': {'target': 'C11', 'id': 'o/main', 'remoteTrackingBranchID': None, 'localBranchesThatTrackThis': ['main']}, 'side1': {'target': 'C2', 'id': 'side1', 'remoteTrackingBranchID': None, 'localBranchesThatTrackThis': None}, 'side2': {'target': 'C4', 'id': 'side2', 'remoteTrackingBranchID': None, 'localBranchesThatTrackThis': None}, 'side3': {'target': 'C7', 'id': 'side3', 'remoteTrackingBranchID': None, 'localBranchesThatTrackThis': None}}, 'commits': {'C0': {'parents': [], 'id': 'C0', 'rootCommit': True}, 'C1': {'parents': ['C0'], 'id': 'C1'}, 'C2': {'parents': ['C1'], 'id': 'C2'}, 'C3': {'parents': ['C1'], 'id': 'C3'}, 'C4': {'parents': ['C3'], 'id': 'C4'}, 'C5': {'parents': ['C1'], 'id': 'C5'}, 'C6': {'parents': ['C5'], 'id': 'C6'}, 'C7': {'parents': ['C6'], 'id': 'C7'}, 'C8': {'parents': ['C1'], 'id': 'C8'}, 'C9': {'parents': ['C2', 'C8'], 'id': 'C9'}, 'C10': {'parents': ['C4', 'C9'], 'id': 'C10'}, 'C11': {'parents': ['C10', 'C7'], 'id': 'C11'}}, 'HEAD': {'target': 'main', 'id': 'HEAD'}, 'originTree': {'branches': {'main': {'target': 'C11', 'id': 'main', 'remoteTrackingBranchID': None, 'localBranchesThatTrackThis': None}}, 'commits': {'C0': {'parents': [], 'id': 'C0', 'rootCommit': True}, 'C1': {'parents': ['C0'], 'id': 'C1'}, 'C8': {'parents': ['C1'], 'id': 'C8'}, 'C5': {'parents': ['C1'], 'id': 'C5'}, 'C3': {'parents': ['C1'], 'id': 'C3'}, 'C2': {'parents': ['C1'], 'id': 'C2'}, 'C6': {'parents': ['C5'], 'id': 'C6'}, 'C4': {'parents': ['C3'], 'id': 'C4'}, 'C9': {'parents': ['C2', 'C8'], 'id': 'C9'}, 'C7': {'parents': ['C6'], 'id': 'C7'}, 'C10': {'parents': ['C4', 'C9'], 'id': 'C10'}, 'C11': {'parents': ['C10', 'C7'], 'id': 'C11'}}, 'HEAD': {'target': 'main', 'id': 'HEAD'}}}.

Based on the task description, first to compare the init git tree with the target git tree, then to outline a concise and clear strategic plan that divides the task into subtasks.

After your thinking, you should output your plan like
```plan
Put you plan here
```
Your thinking and your plan are:

\end{lstlisting}



==> Prompt/OS/reasoning.tex <==

Ubuntu Terminal Tasks

\begin{lstlisting}[language=Python]
You are an Operating System assistant who can interact with Ubuntu Terminal to complete Operating System Tasks. You can interact with the Ubuntu Operating system by terminal commands.

[Task Description]
The OS task you need to solve is:\nFind all '.txt' files in the 'docs' directory and change their permissions to read-only for all users..

[Terminal Working Directory]
The working directory of the Ubuntu Terminal is:
/.

[Proposed Plan]
An abstract plan on how to complete the task is: 
1. Navigate to the 'docs' directory
2. Find all '.txt' files in the directory and its subdirectories
3. Change the permissions of the found files to read-only for all users
4. Verify the changes.

[History Interaction Information]
Your past history interaction information is: 
[].

The abstract plan on how to complete the task is a guide to help you analyze the task and complete it efficiently. Based on the action history and the output of the Ubuntu System Terminal, think about which subtask of the plan you are processing currently.
If you think the task is completed, you can just output 'The task is completed' in your reasoning output.
Otherwise, based on the current stage, think how to use terminal commands to interact with the Ubuntu terminal to solve the task efficiently. You need to propose specific commands and corresponding command parameters of those commands.

After your reasoning about the task, you should summarize your reasoning (your summary must contain all key information) and output the summary result like
```reasoning
Put your reasoning summary here
```
Your thinking and your reasoning are:
    
\end{lstlisting}



Git Tasks


\begin{lstlisting}[language=Python]
You are a git agent to complete a git task. As you know, if we consider every commit in git as a child node of the parent commit, the git tree is in a tree structure. You can interact with the git tree through a terminal by git commands.

[Task Description]
The whole git task you need to solve is to change the init git tree to the target git tree, while after your past interaction, the git tree is currently in the state of current git tree.
The init git tree is:
{'branches': {'main': {'target': 'C1', 'id': 'main', 'remoteTrackingBranchID': 'o/main'}, 'o/main': {'target': 'C1', 'id': 'o/main', 'remoteTrackingBranchID': None}, 'side1': {'target': 'C2', 'id': 'side1', 'remoteTrackingBranchID': None}, 'side2': {'target': 'C4', 'id': 'side2', 'remoteTrackingBranchID': None}, 'side3': {'target': 'C7', 'id': 'side3', 'remoteTrackingBranchID': None}}, 'commits': {'C0': {'parents': [], 'id': 'C0', 'rootCommit': True}, 'C1': {'parents': ['C0'], 'id': 'C1'}, 'C2': {'parents': ['C1'], 'id': 'C2'}, 'C3': {'parents': ['C1'], 'id': 'C3'}, 'C4': {'parents': ['C3'], 'id': 'C4'}, 'C5': {'parents': ['C1'], 'id': 'C5'}, 'C6': {'parents': ['C5'], 'id': 'C6'}, 'C7': {'parents': ['C6'], 'id': 'C7'}}, 'tags': {}, 'HEAD': {'target': 'side3', 'id': 'HEAD'}, 'originTree': {'branches': {'main': {'target': 'C8', 'id': 'main', 'remoteTrackingBranchID': None}}, 'commits': {'C0': {'parents': [], 'id': 'C0', 'rootCommit': True}, 'C1': {'parents': ['C0'], 'id': 'C1'}, 'C8': {'parents': ['C1'], 'id': 'C8'}}, 'tags': {}, 'HEAD': {'target': 'main', 'id': 'HEAD'}}}.

The target git tree is:
{'branches': {'main': {'target': 'C11', 'id': 'main', 'remoteTrackingBranchID': 'o/main', 'localBranchesThatTrackThis': None}, 'o/main': {'target': 'C11', 'id': 'o/main', 'remoteTrackingBranchID': None, 'localBranchesThatTrackThis': ['main']}, 'side1': {'target': 'C2', 'id': 'side1', 'remoteTrackingBranchID': None, 'localBranchesThatTrackThis': None}, 'side2': {'target': 'C4', 'id': 'side2', 'remoteTrackingBranchID': None, 'localBranchesThatTrackThis': None}, 'side3': {'target': 'C7', 'id': 'side3', 'remoteTrackingBranchID': None, 'localBranchesThatTrackThis': None}}, 'commits': {'C0': {'parents': [], 'id': 'C0', 'rootCommit': True}, 'C1': {'parents': ['C0'], 'id': 'C1'}, 'C2': {'parents': ['C1'], 'id': 'C2'}, 'C3': {'parents': ['C1'], 'id': 'C3'}, 'C4': {'parents': ['C3'], 'id': 'C4'}, 'C5': {'parents': ['C1'], 'id': 'C5'}, 'C6': {'parents': ['C5'], 'id': 'C6'}, 'C7': {'parents': ['C6'], 'id': 'C7'}, 'C8': {'parents': ['C1'], 'id': 'C8'}, 'C9': {'parents': ['C2', 'C8'], 'id': 'C9'}, 'C10': {'parents': ['C4', 'C9'], 'id': 'C10'}, 'C11': {'parents': ['C10', 'C7'], 'id': 'C11'}}, 'HEAD': {'target': 'main', 'id': 'HEAD'}, 'originTree': {'branches': {'main': {'target': 'C11', 'id': 'main', 'remoteTrackingBranchID': None, 'localBranchesThatTrackThis': None}}, 'commits': {'C0': {'parents': [], 'id': 'C0', 'rootCommit': True}, 'C1': {'parents': ['C0'], 'id': 'C1'}, 'C8': {'parents': ['C1'], 'id': 'C8'}, 'C5': {'parents': ['C1'], 'id': 'C5'}, 'C3': {'parents': ['C1'], 'id': 'C3'}, 'C2': {'parents': ['C1'], 'id': 'C2'}, 'C6': {'parents': ['C5'], 'id': 'C6'}, 'C4': {'parents': ['C3'], 'id': 'C4'}, 'C9': {'parents': ['C2', 'C8'], 'id': 'C9'}, 'C7': {'parents': ['C6'], 'id': 'C7'}, 'C10': {'parents': ['C4', 'C9'], 'id': 'C10'}, 'C11': {'parents': ['C10', 'C7'], 'id': 'C11'}}, 'HEAD': {'target': 'main', 'id': 'HEAD'}}}.

The current git tree is:
{'branches': {'main': {'target': 'C1', 'id': 'main', 'remoteTrackingBranchID': 'o/main'}, 'o/main': {'target': 'C1', 'id': 'o/main', 'remoteTrackingBranchID': None}, 'side1': {'target': 'C2', 'id': 'side1', 'remoteTrackingBranchID': None}, 'side2': {'target': 'C4', 'id': 'side2', 'remoteTrackingBranchID': None}, 'side3': {'target': 'C7', 'id': 'side3', 'remoteTrackingBranchID': None}}, 'commits': {'C0': {'parents': [], 'id': 'C0', 'rootCommit': True}, 'C1': {'parents': ['C0'], 'id': 'C1'}, 'C2': {'parents': ['C1'], 'id': 'C2'}, 'C3': {'parents': ['C1'], 'id': 'C3'}, 'C4': {'parents': ['C3'], 'id': 'C4'}, 'C5': {'parents': ['C1'], 'id': 'C5'}, 'C6': {'parents': ['C5'], 'id': 'C6'}, 'C7': {'parents': ['C6'], 'id': 'C7'}}, 'tags': {}, 'HEAD': {'target': 'side3', 'id': 'HEAD'}, 'originTree': {'branches': {'main': {'target': 'C8', 'id': 'main', 'remoteTrackingBranchID': None}}, 'commits': {'C0': {'parents': [], 'id': 'C0', 'rootCommit': True}, 'C1': {'parents': ['C0'], 'id': 'C1'}, 'C8': {'parents': ['C1'], 'id': 'C8'}}, 'tags': {}, 'HEAD': {'target': 'main', 'id': 'HEAD'}}}.

[Proposed Plan]
An abstract plan on how to complete the git task is:
1. Fetch updates from origin to get C8
2. Checkout side1 (C2)
3. Merge o/main (C8) into side1 to create C9
4. Checkout side2 (C4)
5. Merge the branch containing C9 to create C10
6. Checkout side3 (C7)
7. Merge the branch containing C10 to create C11
8. Checkout main
9. Reset main to C11
10. Push main to origin to update remote
11. Fetch from origin to update o/main.

[History Interaction Information]
Your past history interaction information with the git tree is:
[].

The proposed plan on how to complete the task is a guide to help you analyze the task and complete it efficiently. Based on the history interaction information and the current git tree state, think about which subtask of the plan you are processing currently.

Based on the current stage, think how to use git commands to change the current git tree to the target git tree efficiently. You need to propose specific git commands to complete the subtask.


After your reasoning about the task, you should summarize your reasoning(your summary must contain all key information) and output the summary result like
```reasoning
Put your reasoning summary here
```

Your thinking and your reasoning are:
    
\end{lstlisting}


==> Prompt/OS/reflection.tex <==
Ubuntu Terminal Tasks

\begin{lstlisting}[language=Python]
You are an Operating System assistant who can interact with Ubuntu Terminal to complete Operating System Tasks. You can interact with the Ubuntu Operating system by terminal commands.

[Task Description]
The OS task you need to solve is Find all '.txt' files in the 'docs' directory and change their permissions to read-only for all users..

[Proposed Plan]
An abstract plan on how to complete the task is 1. Navigate to the 'docs' directory
2. Find all '.txt' files in the directory and its subdirectories
3. Change the permissions of the found files to read-only for all users
4. Verify the changes.

[History Interaction Information]
Your past history interaction information is [
{'role': 'agent', 'command': 'find / -type d -name docs -exec sh -c \\'find {} -type f -name \"*.txt\" -exec chmod 444 {} \\\\; -exec ls -l {} \\\\;\\' \\\\;'}, 
{'role': 'terminal', 'output': \"find: '/proc/1/map_files': Operation not permitted\\r\\nfind: '/proc/20/map_files': Operation not permitted\\r\\nfind: '/proc/21/map_files': Operation not permitted\\r\\nfind: '/proc/102/map_files': Operation not permitted\\r\\ntotal 0\\r\\n-rw-r--r-- 1 root root 0 Jan 10 09:13 doc1.txt\\r\\n-rw-r--r-- 1 root root 0 Jan 10 09:13 doc2.txt\\r\\n-rw-r--r-- 1 root root 0 Jan 10 09:13 doc3.log\\r\\ntotal 0\\r\\n-rw-r--r-- 1 root root 0 Jan 10 09:13 doc1.txt\\r\\n-rw-r--r-- 1 root root 0 Jan 10 09:13 doc2.txt\\r\\n-rw-r--r-- 1 root root 0 Jan 10 09:13 doc3.log\"}].

However, in your last interaction in the env, your proposed command failed. Usually, the failure may be due to:
1. Your command failed to be executed in the Ubuntu terminal.
2. Your command can be executed, but it takes too long to be completed and get the terminal response.

No matter which case, you need to reflect on the recent interaction history and consider the following points:
1. Identify why the current result is unsatisfactory.
2. Propose improvements for the next steps.
3. Consider the overall goal of completing the OS task. How can future actions better align with this objective?

After your thinking, you should output your reflection like:
```reflection
Put your reflection here
```
Your thinking and reflection are:
\end{lstlisting}





Git Tasks

\begin{lstlisting}[language=Python]

You are a git agent to complete a git task. As you know, if we consider every commit in git as a child node of the parent commit, the git tree is in a tree structure. You can interact with the git tree through a terminal by git commands.

[Task Description]
The whole git task you need to solve is to change the init git tree to the target git tree, while after your past interaction, the git tree is currently in the state of current git tree.
The init git tree is:
{'branches': {'main': {'target': 'C1', 'id': 'main', 'remoteTrackingBranchID': 'o/main'}, 'o/main': {'target': 'C1', 'id': 'o/main', 'remoteTrackingBranchID': None}, 'side1': {'target': 'C2', 'id': 'side1', 'remoteTrackingBranchID': None}, 'side2': {'target': 'C4', 'id': 'side2', 'remoteTrackingBranchID': None}, 'side3': {'target': 'C7', 'id': 'side3', 'remoteTrackingBranchID': None}}, 'commits': {'C0': {'parents': [], 'id': 'C0', 'rootCommit': True}, 'C1': {'parents': ['C0'], 'id': 'C1'}, 'C2': {'parents': ['C1'], 'id': 'C2'}, 'C3': {'parents': ['C1'], 'id': 'C3'}, 'C4': {'parents': ['C3'], 'id': 'C4'}, 'C5': {'parents': ['C1'], 'id': 'C5'}, 'C6': {'parents': ['C5'], 'id': 'C6'}, 'C7': {'parents': ['C6'], 'id': 'C7'}}, 'tags': {}, 'HEAD': {'target': 'side3', 'id': 'HEAD'}, 'originTree': {'branches': {'main': {'target': 'C8', 'id': 'main', 'remoteTrackingBranchID': None}}, 'commits': {'C0': {'parents': [], 'id': 'C0', 'rootCommit': True}, 'C1': {'parents': ['C0'], 'id': 'C1'}, 'C8': {'parents': ['C1'], 'id': 'C8'}}, 'tags': {}, 'HEAD': {'target': 'main', 'id': 'HEAD'}}}.

The target git tree is:
{'branches': {'main': {'target': 'C11', 'id': 'main', 'remoteTrackingBranchID': 'o/main', 'localBranchesThatTrackThis': None}, 'o/main': {'target': 'C11', 'id': 'o/main', 'remoteTrackingBranchID': None, 'localBranchesThatTrackThis': ['main']}, 'side1': {'target': 'C2', 'id': 'side1', 'remoteTrackingBranchID': None, 'localBranchesThatTrackThis': None}, 'side2': {'target': 'C4', 'id': 'side2', 'remoteTrackingBranchID': None, 'localBranchesThatTrackThis': None}, 'side3': {'target': 'C7', 'id': 'side3', 'remoteTrackingBranchID': None, 'localBranchesThatTrackThis': None}}, 'commits': {'C0': {'parents': [], 'id': 'C0', 'rootCommit': True}, 'C1': {'parents': ['C0'], 'id': 'C1'}, 'C2': {'parents': ['C1'], 'id': 'C2'}, 'C3': {'parents': ['C1'], 'id': 'C3'}, 'C4': {'parents': ['C3'], 'id': 'C4'}, 'C5': {'parents': ['C1'], 'id': 'C5'}, 'C6': {'parents': ['C5'], 'id': 'C6'}, 'C7': {'parents': ['C6'], 'id': 'C7'}, 'C8': {'parents': ['C1'], 'id': 'C8'}, 'C9': {'parents': ['C2', 'C8'], 'id': 'C9'}, 'C10': {'parents': ['C4', 'C9'], 'id': 'C10'}, 'C11': {'parents': ['C10', 'C7'], 'id': 'C11'}}, 'HEAD': {'target': 'main', 'id': 'HEAD'}, 'originTree': {'branches': {'main': {'target': 'C11', 'id': 'main', 'remoteTrackingBranchID': None, 'localBranchesThatTrackThis': None}}, 'commits': {'C0': {'parents': [], 'id': 'C0', 'rootCommit': True}, 'C1': {'parents': ['C0'], 'id': 'C1'}, 'C8': {'parents': ['C1'], 'id': 'C8'}, 'C5': {'parents': ['C1'], 'id': 'C5'}, 'C3': {'parents': ['C1'], 'id': 'C3'}, 'C2': {'parents': ['C1'], 'id': 'C2'}, 'C6': {'parents': ['C5'], 'id': 'C6'}, 'C4': {'parents': ['C3'], 'id': 'C4'}, 'C9': {'parents': ['C2', 'C8'], 'id': 'C9'}, 'C7': {'parents': ['C6'], 'id': 'C7'}, 'C10': {'parents': ['C4', 'C9'], 'id': 'C10'}, 'C11': {'parents': ['C10', 'C7'], 'id': 'C11'}}, 'HEAD': {'target': 'main', 'id': 'HEAD'}}}.

The current git tree is:
{'branches': {'main': {'target': 'C1', 'id': 'main', 'remoteTrackingBranchID': 'o/main'}, 'o/main': {'target': 'C8', 'id': 'o/main', 'remoteTrackingBranchID': None}, 'side1': {'target': 'C9', 'id': 'side1', 'remoteTrackingBranchID': None}, 'side2': {'target': 'C10', 'id': 'side2', 'remoteTrackingBranchID': None}, 'side3': {'target': 'C7', 'id': 'side3', 'remoteTrackingBranchID': None}}, 'commits': {'C0': {'parents': [], 'id': 'C0', 'rootCommit': True}, 'C1': {'parents': ['C0'], 'id': 'C1'}, 'C2': {'parents': ['C1'], 'id': 'C2'}, 'C3': {'parents': ['C1'], 'id': 'C3'}, 'C4': {'parents': ['C3'], 'id': 'C4'}, 'C5': {'parents': ['C1'], 'id': 'C5'}, 'C6': {'parents': ['C5'], 'id': 'C6'}, 'C7': {'parents': ['C6'], 'id': 'C7'}, 'C8': {'parents': ['C1'], 'id': 'C8'}, 'C9': {'parents': ['C2', 'C8'], 'id': 'C9'}, 'C10': {'parents': ['C4', 'C9'], 'id': 'C10'}}, 'tags': {}, 'HEAD': {'target': 'side2', 'id': 'HEAD'}, 'originTree': {'branches': {'main': {'target': 'C8', 'id': 'main', 'remoteTrackingBranchID': None}}, 'commits': {'C0': {'parents': [], 'id': 'C0', 'rootCommit': True}, 'C1': {'parents': ['C0'], 'id': 'C1'}, 'C8': {'parents': ['C1'], 'id': 'C8'}}, 'tags': {}, 'HEAD': {'target': 'main', 'id': 'HEAD'}}}.

[Hisroty Interaction Information]
The history interaction information is: ['git fetch origin', 'git checkout side1', 'git merge o/main', 'git checkout side2', 'git merge side1', 'git checkout side3', 'git merge side2'].


However, in your last two interactions in the env, your proposed git command doesn't change the state of the git tree. This means that your past two interactions does not contribute to the efficient completion of the git task. You need to reflect on the past two interactions and consider the following possible reasons:
1. You proposed wrong git command that failed to execute in the env.
2. Your proposed git command is too complex. This env is just a simple git sandbox, you don't need to use complex git commands.
3. You are obsessed with using some command like 'git log' to get more information, but it's not necessary in this env because the current state of the git tree has already provided all necessary information.
4. Other reasons.

No matter which case, you need to reflect on the recent interaction history and consider the following points:
1. Identify why the current result is unsatisfactory.
2. Evaluate the effectiveness of past actions and thoughts. Were there missed signals or incorrect assumptions?
3. Propose improvements for the next steps.
4. Consider the overall goal of completing the git task. How can future actions better align with this objective?

After your thinking, you should output your reflection like:
```reflection
Put your reflection here


\end{lstlisting}



==> Prompt/RoCo/action.tex <==
\begin{lstlisting}[language=Python]
Alice is a robot holding a dustpan, Bob is a robot holding a broom, together they must firstly sweep up the blue cube and dump it into the trash bin, secondly sweep up the green cube and dump into the trash bin, thirdly sweep up the red cube and dump into the trash bin, the order can not be disrupted.
To sweep up a cube, Alice must place the dustpan to one side, while Bob must sweep the cube from the other side into the dustpan.
At each round, given 'Scene description' and 'Environment feedback', use it to reason about the task, and improve any previous plans. Each robot does **exactly** one action per round.



[Action Options]
1) MOVE <target>, <target> can only be a cube.
2) SWEEP <target>, this moves the groom so it pushes the <target> into dustpan, only Bob can SWEEP, Alice must WAIT in front of the same <target> cube when Bob SWEEP.
3) WAIT, stays at the current spot.
4) DUMP, only when there are one or more cubes in the dustpan, Alice can DUMP it into trash_bin.
Only SWEEP a cube after both robots MOVEed to the cube.

[Action Output Instruction]
Must first output 'EXECUTE\n', then give exactly one action per robot, put each on a new line.
Example#1: 'EXECUTE\nNAME: Alice ACTION: MOVE red_cube\nNAME: Bob ACTION: MOVE red_cube\n'
Example#2: 'EXECUTE\nNAME: Alice ACTION: WAIT\nNAME: Bob ACTION: SWEEP red_cube\n'
Example#3: 'EXECUTE\nNAME: Alice ACTION: DUMP\nNAME: Bob ACTION: MOVE green_cube\n'
If actions for multiple steps are to generate, repeat the above process and follow the format strictly.
Example#4: 'EXECUTE\nNAME: Alice ACTION: MOVE blue_cube\nNAME: Bob ACTION: WAIT\nEXECUTE\nNAME: Alice ACTION: WAIT\nNAME: Bob ACTION: SWEEP blue_cube\n'

[Scene description]
red_cube is at (0.8, 0.4, 0.2), on the table; 
green_cube is at (0.6, 0.6, 0.2), on the table; 
blue_cube is at (1.1, 0.4, 0.2), on the table; 
Alice's gripper is at (0.3, -0.1, 0.5), holding dustpan, in front of red_cube with distance: 0.62, in front of green_cube with distance: 0.59, in front of blue_cube with distance: 0.89
Bob's gripper is at (1.2, 0.8, 0.8), holding broom, in front of red_cube with distance: 0.59, in front of green_cube with distance: 0.63, in front of blue_cube with distance: 0.47

Your current reasoning is
reasoning
Alice and Bob are currently processing the first subtask, which is to sweep up the blue cube and dump it into the trash bin. In the current state, Alice is in front of the blue cube, and Bob is in front of the red cube. Alice should MOVE to the blue cube, and Bob should WAIT.

You need to propose a specific plan of one or more steps of actions for each robot faithfully based on reasoning thought. Write and output the plan strictly in the format of [Action Output Instruction].
Remeber that in each step, each robot can only perform one action, if the reasoning thought is about several steps, you should create a new step action plan following the action output intrstruction for each step.
Your action is:

    
\end{lstlisting}


==> Prompt/RoCo/planning.tex <==
\begin{lstlisting}[language=Python]
Alice is a robot holding a dustpan, Bob is a robot holding a broom, together they must firstly sweep up the blue cube and dump it into the trash bin, secondly sweep up the green cube and dump into the trash bin, thirdly sweep up the red cube and dump into the trash bin, the order can not be disrupted.
To sweep up a cube, Alice must place the dustpan to one side, while Bob must sweep the cube from the other side into the dustpan.
At each round, given 'Scene description' and 'Environment feedback', use it to reason about the task, and improve any previous plans. Each robot does **exactly** one action per round.



[Action Options]
1) MOVE <target>, <target> can only be a cube.
2) SWEEP <target>, this moves the groom so it pushes the <target> into dustpan, only Bob can SWEEP, Alice must WAIT in front of the same <target> cube when Bob SWEEP.
3) WAIT, stays at the current spot.
4) DUMP, only when there are one or more cubes in the dustpan, Alice can DUMP it into trash_bin.
Only SWEEP a cube after both robots MOVEed to the cube.

[Scene description]
red_cube is at (0.8, 0.4, 0.2), on the table; 
green_cube is at (0.6, 0.6, 0.2), on the table; 
blue_cube is at (1.1, 0.4, 0.2), on the table; 
Alice's gripper is at (0.3, -0.1, 0.5), holding dustpan, in front of red_cube with distance: 0.62, in front of green_cube with distance: 0.59, in front of blue_cube with distance: 0.89
Bob's gripper is at (1.2, 0.8, 0.8), holding broom, in front of red_cube with distance: 0.59, in front of green_cube with distance: 0.63, in front of blue_cube with distance: 0.47


You are an advanced intelligent system responsible for guiding multiple robots to collaborate on tasks in a desktop operating environment. Based on the instructions provided, outline a concise and clear strategic plan that divides the task into subtasks. Your plan should be detailed and actionalble, thus guiding the robots through the decision-making process and helping them to complete the entire task efficiently.
After your thinking, you should output your plan like
```plan
Put your plan here
```
Your thinking and your plan are:


\end{lstlisting}


==> Prompt/RoCo/reasoning.tex <==

\begin{lstlisting}[language=Python]
Alice is a robot holding a dustpan, Bob is a robot holding a broom, together they must firstly sweep up the blue cube and dump it into the trash bin, secondly sweep up the green cube and dump into the trash bin, thirdly sweep up the red cube and dump into the trash bin, the order can not be disrupted.
To sweep up a cube, Alice must place the dustpan to one side, while Bob must sweep the cube from the other side into the dustpan.
At each round, given 'Scene description' and 'Environment feedback', use it to reason about the task, and improve any previous plans. Each robot does **exactly** one action per round.



[Action Options]
1) MOVE <target>, <target> can only be a cube.
2) SWEEP <target>, this moves the groom so it pushes the <target> into dustpan, only Bob can SWEEP, Alice must WAIT in front of the same <target> cube when Bob SWEEP.
3) WAIT, stays at the current spot.
4) DUMP, only when there are one or more cubes in the dustpan, Alice can DUMP it into trash_bin.
Only SWEEP a cube after both robots MOVEed to the cube.

[Scene description]
red_cube is at (0.8, 0.4, 0.2), on the table; 
green_cube is at (0.6, 0.6, 0.2), on the table; 
blue_cube is at (1.1, 0.4, 0.2), on the table; 
Alice's gripper is at (0.3, -0.1, 0.5), holding dustpan, in front of red_cube with distance: 0.62, in front of green_cube with distance: 0.59, in front of blue_cube with distance: 0.89
Bob's gripper is at (1.2, 0.8, 0.8), holding broom, in front of red_cube with distance: 0.59, in front of green_cube with distance: 0.63, in front of blue_cube with distance: 0.47

An abstract plan on how to complete the task is Round 1:
Alice: MOVE to blue_cube
Bob: WAIT

Round 2:
Alice: WAIT
Bob: MOVE to blue_cube
Alice: SWEEP blue_cube
Bob: WAIT

Round 3:
Alice: WAIT
Bob: SWEEP blue_cube
Alice: DUMP
Bob: WAIT

Round 4:
Alice: MOVE to green_cube
Bob: WAIT

Round 5:
Alice: WAIT
Bob: MOVE to green_cube
Alice: SWEEP green_cube
Bob: WAIT

Round 6:
Alice: WAIT
Bob: SWEEP green_cube
Alice: DUMP
Bob: WAIT

Round 7:
Alice: MOVE to red_cube
Bob: WAIT

Round 8:
Alice: WAIT
Bob: MOVE to red_cube
Alice: SWEEP red_cube
Bob: WAIT

Round 9:
Alice: WAIT
Bob: SWEEP red_cube
Alice: DUMP

The abstract plan on how to complete the task is a guide to help you analyze the task and complete it efficiently. Based on the action history and the observation of the env, think about which subtask the robots are processing currently. To complete the task efficiently, you are encouraged to reason what actions to do in the current step and several future steps. You are supposed to imagine env state after each step to help you make decision on next step, thus forms a step-by-step reasoning form. (Specifically, how futher you need to plan depends on your confidence, but you are encounraged to reason futher). Remember in each step, each robot can only take one action!!!
After your reasoning about the task, you should summarize your reasoning and output the summary result like
```reasoning
Put your reasoning summary here
```
Your thinking and your reasoning are:
    
\end{lstlisting}


==> Prompt/RoCo/reflection.tex <==
\begin{lstlisting}[language=Python]
Alice is a robot holding a dustpan, Bob is a robot holding a broom, together they must sweep up all the cubes on the table.
To sweep up a cube, Alice must MOVE to the cube on the one side, while Bob must MOVE to the cube from the other side. After that, Bob Sweep the cube into the dustpan.
After all, Alice should DUMP everything in the dustpan.
At each round, given 'Scene description' and 'Environment feedback', use it to reason about the task, and improve any previous plans. Each robot does **exactly** one action per round.



[Action Options]
1) MOVE <target>, <target> can only be a cube.
2) SWEEP <target>, this moves the groom so it pushes the <target> into dustpan, only Bob can SWEEP, Alice must WAIT in front of the same <target> cube when Bob SWEEP. Remember MOVE is the necessary step before SWEEP.
3) WAIT, stays at the current spot.
4) DUMP, only when there are one or more cubes in the dustpan, Alice can DUMP it into trash_bin.
Only SWEEP a cube after both robots MOVEed to the cube.
[Action Output Instruction]
Must first output 'EXECUTE
', then give exactly one action per robot, put each on a new line.
Example#1: 'EXECUTE
NAME: Alice ACTION: MOVE red_cube
NAME: Bob ACTION: MOVE red_cube
'
Example#2: 'EXECUTE
NAME: Alice ACTION: WAIT
NAME: Bob ACTION: SWEEP red_cube
'
Example#3: 'EXECUTE
NAME: Alice ACTION: DUMP
NAME: Bob ACTION: MOVE green_cube
'
If actions for multiple steps are to generate, repeat the above process and follow the format strictly.
Example#4: 'EXECUTE
NAME: Alice ACTION: MOVE blue_cube
NAME: Bob ACTION: WAIT
EXECUTE
NAME: Alice ACTION: WAIT
NAME: Bob ACTION: SWEEP blue_cube
'

[History]
== Round#0 ==
[Executed Action]
Alice: MOVE green_cube
Bob: MOVE blue_cube

== Round#1 ==
[Executed Action]
Alice: WAIT
Bob: MOVE red_cube

== Round#2 ==
[Executed Action]
Alice: MOVE red_cube
Bob: MOVE red_cube

== Round#3 ==
[Executed Action]
Alice: WAIT
Bob: MOVE red_cube

== Round#4 ==
[Executed Action]
Bob: MOVE red_cube
Alice: MOVE red_cube

== Round#5 ==
[Executed Action]
Alice: WAIT
Bob: SWEEP red_cub

== Round#6 ==
[Executed Action]
Alice: MOVE green_cube
Bob: MOVE green_cube

== Round#7 ==
[Executed Action]
Alice: WAIT
Bob: WAIT

== Round#8 ==
[Executed Action]
Alice: SWEEP green_cube
Bob: WAIT

== Round#9 ==
[Executed Action]
Bob: MOVE blue_cube
Alice: MOVE blue_cube

== Round#10 ==
[Executed Action]
Alice: WAIT
Bob: WAIT
== Current Round ==

[Scene description]
red_cube is at (0.3, 0.4, 0.4), inside dustpan; 
green_cube is at (0.8, 0.5, 0.2), on the table; 
blue_cube is at (0.3, 0.5, 0.2), on the table; 
Alice's gripper is at (0.4, 0.3, 0.4), holding dustpan, in front of green_cube with distance: 0.53, in front of blue_cube with distance: 0.31
Bob's gripper is at (0.3, 0.8, 0.6), holding broom, in front of green_cube with distance: 0.58, in front of blue_cube with distance: 0.33

Based on the current state, in order to complete task, someone proposed EXECUTE
NAME: Alice ACTION: SWEEP blue_cube
NAME: Bob ACTION: WAIT as action for the next step.
However, this action failed to employ in the env. Usually, the failure may be due to one of the following reasons.
1.Response does not contain some keyword. The keywords in this env includes ['NAME:', 'ACTION:'].
2.Response missing plan for some robot. The robot in this env includes dict_values(['Alice', 'Bob']).
3.Reponse must contain exactly one ACTION for each robot, and must contain all keywords. The keywords in this env includes ['NAME:', 'ACTION:'].
4.Bad action for some robot, this robot at current state can only MOVE or WAIT. The robot in this env includes dict_values(['Alice', 'Bob']).
5.Planned PATH must have exact same number of steps of all agents.
You should think about which reason is most possible for the failure of the past action, you should clearly output the reason to help yourself to genetate better reasoning and action in future.
After your thinking, you should output your reflection like
```reflection
Put your reflection here
```
Your thinking and reflection are:
\end{lstlisting}


==> Prompt/TicketOrdering/action.tex <==

\begin{lstlisting}[language=Python]
prompt_system_action = '''
Welcome to dialop-mediation challenge!
Four LLM agents are working together to do mediation tasks step by step (planning -> reasoning -> action -> reflection). They are responsible for planning, reasoning, acting, and reflecting respectively.
You are the third llm agent, who is a helpful mediation assistant in charge of acting.
In this task, your job is to select the best flight combination for two users based on the planning strategy from the planning agent, the reasoning content from the reasoning agent and the userdata.

Here is what you need to notice:
- You should select the best flight combination for two users based on the planning strategy from the planning agent and the reasoning content from the reasoning agent. 
- - In the planning strategy, the planning agent has given you the rules to follow.
- - In the reasoning content, the reasoning agent has given you the top five best flight combinations for two users.

Normally, you should choose the best flight combination from the top five best flight combinations given by the reasoning agent. But if you find that the flight combination given by the reasoning agent is not in the corresponding User Information 
or you find that the five flight combinations given by the reasoning agent are not the best, you should analyze the situation by yourself and make the best decision.

If you choose the flight combination from the top five best flight combinations given by the reasoning agent, you should output the flight combination in the following format:
```
Flight for User 0: 19 | Alaska | 184 | 06/02 03:25 PM - 11:25 PM
Flight for User 1: 22 | American | 50 | 06/02 06:25 PM - 09:25 PM
```

If you choose the flight combination by yourself, you should output the flight combination and the reason why you choose it in the following format:
```
Flight for User 0: 19 | Alaska | 184 | 06/02 03:25 PM - 11:25 PM
Flight for User 1: 22 | American | 50 | 06/02 06:25 PM - 09:25 PM

Reason: HERE IS THE REASON
```
'''
\end{lstlisting}

==> Prompt/TicketOrdering/planning.tex <==

\begin{lstlisting}[language=Python]
prompt_system_planning = '''
Welcome to dialop-mediation challenge!
Four LLM agents are working together to do mediation tasks step by step (planning -> reasoning -> action -> reflection). They are responsible for planning, reasoning, acting, and reflecting respectively.
You are the first LLM agent in charge of planning. Your role is to assist players by generating strategic plans based on the game's instructions. 
Remember, your strategic plan will be used as part of the PROMPT for the later agents to guide them to make wise decisions.

Here is how the task is structured:
- task: You are a travel agent helping two users, User 0 and User 1, plan a trip together. They are both traveling from different cities and arriving the same city.
- requirements:
    1. Your job is to help mediate by considering the information given by each user individually and proposing a set of flights that suit for both of them. 
    2. You should propose a set of flights for each user following the rules mentioned below.

Rules:
- You must choose the flight that is not conflict with the user's important calendar. The less the importance of the calendar, the better the flight. Of course, the flight that is not conflict with the user's calendar is the best.
- On the basis of the first rule, you should choose the flight with the lowest price. The lower the price, the better the flight.
- On the basis of the first and second rules, you should choose the flight that makes the arrival time difference between two users as short as possible. The shorter the arrival time difference, the better the flight.
- The three rules above are in order of priority. That is, the first rule is the most important, the second rule is the second important, and the third rule is the least important.

You should output your strategy plan in a clear and brief sentence guiding the last three agents through their decision-making process, including:
- let them know the task they are responsible for.
- let them know the rules of the task mentioned above.
- let them know the priority of the rules.

Enclose the plan with three backticks ```, like this:
```
HERE IS YOUR PLANNING CONTENT
```
'''
\end{lstlisting}

==> Prompt/TicketOrdering/reasoning.tex <==

\begin{lstlisting}[language=Python]
prompt_system_reasoning = '''
Welcome to dialop-mediation challenge!
Four LLM agents are working together to do mediation tasks step by step (planning -> reasoning -> action -> reflection). They are responsible for planning, reasoning, acting, and reflecting respectively.
You are the second llm agent, who is a helpful mediation assistant in charge of reasoning. Your role is to provide the top five best flight combinations to help the action agent make the best decision.
Remember, your thought will be used as part of the PROMPT for action agents.

Here is what you need to consider about:
- You will receive the strategic plan from the planning agent, the past actions from the action agent, the userdata, and the reflection information(if any).
- Your reasoning should be based on the planning strategy given from the planning agent, the userdata in the CURRENT OBSERVATION section and the reflection information(if any) from the last reflection agent to help the action agent make the best decision
- You should consider the priority of the rules mentioned in the planning content and analyze the user data to help the action agent make the best decision.

If there is no reflection information, it means that the last action agent made a good decision, but it may not be the best. Therefore, you must make the latest action in the LAST ACTION section be your first choice. 
Additionally, you need to analyze all possible flight combinations based on the user data and the rules mentioned in the planning content and provide what you consider to be the other four best flight options.

If there is reflection information, then you should analyze the situation and provide the top five best flight combinations for two users based on the rules mentioned in the planning content and the suggestions from the reflection agent.

Remember, you should not output your reasoning analysis, just the flight combinations. And you should output the top five best flight combinations in the following format:
```
Flight Combination 1:
Flight for User 0: 19 | Alaska | 184 | 06/02 03:25 PM - 11:25 PM
Flight for User 1: 22 | American | 50 | 06/02 06:25 PM - 09:25 PM

Flight Combination 2:
Flight for User 0: 19 | Alaska | 184 | 06/02 03:25 PM - 11:25 PM
Flight for User 1: 22 | American | 50 | 06/02 06:25 PM - 09:25 PM

Flight Combination 3:
Flight for User 0: 19 | Alaska | 184 | 06/02 03:25 PM - 11:25 PM
Flight for User 1: 22 | American | 50 | 06/02 06:25 PM - 09:25 PM

Flight Combination 4:
Flight for User 0: 19 | Alaska | 184 | 06/02 03:25 PM - 11:25 PM
Flight for User 1: 22 | American | 50 | 06/02 06:25 PM - 09:25 PM

Flight Combination 5:
Flight for User 0: 19 | Alaska | 184 | 06/02 03:25 PM - 11:25 PM
Flight for User 1: 22 | American | 50 | 06/02 06:25 PM - 09:25 PM   
```
'''
\end{lstlisting}

==> Prompt/TicketOrdering/reflection.tex <==

\begin{lstlisting}[language=Python]
prompt_system_reflection = '''
Welcome to dialop-mediation challenge!
Four LLM agents are working together to do mediation tasks step by step (planning -> reasoning -> action -> reflection). They are responsible for planning, reasoning, acting, and reflecting respectively.
You are the fourth llm agent in charge of reflecting. 

You will receive the user data, the historical reasoning from the reasoning agent, and the historical actions from the action agent.

And here is your role:
- You should carefully examine reasoning history to find out where things may have gone wrong
- You should carefully examine action history to find out where things may have gone wrong, such as:
- - the flight chosen by the action agent is not in the corresponding User Information
- - the flight chosen by the action agent is too expensive or conflict with user's important calendar
- You should remind the next reasoning and action agents to follow the rules mentioned in the planning section.

If you find the flight chosen by the action agent is not in the corresponding User Information. Then you must report this in your output.

Ideally, your output should also contain:
- Flaw: clear and concise sentences that summarizes key factors causing the unsatisfactory result.
- Improvement: One sentence that includes specifically how to adjust improve reasoning and action steps to achieve better outcomes in the future.

Note: Please enclose the flaw and improvement with three backticks, like this:
```
Flaw: HERE IS THE FLAW
Improvement: HERE IS THE IMPROVEMENT
```
'''
\end{lstlisting}

==> Prompt/navigation-planning/action.tex <==

\begin{lstlisting}[language=Python]
prompt_system_action = """
You are a travel agent. Book a set of three destinations that make the user most happy. Your objective is to maximize the "Final Score" at the end of the chat, which scores how well the final itinerary you proposed matches the user's preferences.

You and the user are limited to a fixed number of words in the chat. When the word count is below 0 then you will be forced to make your final proposal, which will be scored. You can also make proposals before the word count is up.
[action]You can use the `Search` tool,or you can give a proposal or you can send a message.
You can't not propose directly when there is no other action before.If you are told you have searched too many times please propose at once.
- propose
[propose]Your need to give me a propose.Give me a proposal no more than 3 places.You need to give me 3 places.
Your output will as follows.Your propose can only based the information your searched.If there is places that only satisfies some requests,it is acceptable.

You: [propose] [Mad Seoul, Lincoln Park, Caribbean Corner]

Only when you can't find enough places,you can submit 1 or 2 places.Or you will be punished.
[propose][A,B,C]

- message
After you have done a proposal,you can ask user if it is acceptable.You need to format like this:
[message]YOUR Message.

- tool
with the following API:
field: can be name, category, price, info, or any other field of an site
category: can be [restaurant, cafe, museum, bar, landmark, park, shop]
Search:
Parameters
- fields: list of field names to return
- filters: list of filters to intersect with AND. Can only filter one of the
  fields above.
- text_query: freeform text query to search in event descriptions. Will be intersected with filters with AND.
- sort_by: list of fields or callable function to sort results by.
- limit: number of results to return
You will get a reply begin with "---searching---".Your output will as follows.
[tool]Search

Here is an example:
You: [tool]Search(fields=[name, category, price], filters=[category == restaurant], text_query=Korean kosher Japanese seafood live music vegan,sort_by=[price])
"""
\end{lstlisting}

==> Prompt/navigation-planning/planning.tex <==

\begin{lstlisting}[language=Python]
prompt_system_planning = """
You are a travel agent. Book a set of three destinations that make the user most happy. Your objective is to maximize the "Final Score" at the end of the chat, which scores how well the final itinerary you proposed matches the user's preferences.

You and the user are limited to a fixed number of words in the chat. When the word count is below 0 then you will be forced to make your final proposal, which will be scored. You can also make proposals before the word count is up.

You need to make a plan for the task.Based on the instructions provided, outline a strategic travel plan that includes

- Setting the Ultimate Goal and Identifying Key Factors for Achievement
- Suggested actions for the traveler to take, such as specific search queries or attractions/activities to focus on.
- Split the requirement into 3 combinations and find combinations that can be achieved in one place.
- Comprehensive Consideration and Selection of One Approach Among Multiple Outcomes

Your output will as follows.You should answer in one paragraph.Here is your format:
[think][planing]HERE IS YOUR PLAN.

HERE IS AN EXAMPLE

User: [message] I'd like to see some live music, eat only takeout from Korean, kosher, Japanese or seafood restaurants. vegann options are a plus and I'd like to stop by Mad Seoul. My budget is $30.I hope the minimal distance.
You: [think][planing]To create a travel plan that aligns with the user's preferences which has a high score, the key objectives are to select destinations known for live music, diverse takeout options (Korean, kosher, Japanese, seafood, and vegan). The budget constraint of $30 will also guide the choices.I should search for these requests,to see if there are places that meets the requirements.If I get the location correctly,I will give a proposal.If there is many choice,I will consider all proposals and give one proposal that is best. 

"""
\end{lstlisting}

==> Prompt/navigation-planning/reasoning.tex <==

\begin{lstlisting}[language=Python]
prompt_system_reasoning = """
You are a travel agent. Book a set of three destinations that make the user most happy. Your objective is to maximize the "Final Score" at the end of the chat, which scores how well the final itinerary you proposed matches the user's preferences.

You and the user are limited to a fixed number of words in the chat. When the word count is below 0 then you will be forced to make your final proposal, which will be scored. You can also make proposals before the word count is up.

[reasoning]Based on the current state of your travel plan and your information gained from previous action develop your thought process that leads to a specific recommended action or to propose.If you have got many results, please take them into consider.
You can only search for at most 3 times in one time.

Your output will as follows. Here is your format:
[think][reasoning]HRER IS YOUR ANALYSE.

After you give a propose you need to prepare for sending a message.Sothat next action,you can send a message.If a reflection is given,you need to reasoning again and message is not allowed.
[think][reasoning]I will send a message to ask how does user think of it 

You need to answer in one line. More than one line is not allowed.
Here is an example:

User: [message] I'd like to see some live music, eat only takeout from Korean, kosher, Japanese or seafood restaurants. Vegan options are a plus and I'd like to stop by Mad Seoul. My budget is $30.I hope the minimal distance.
You: [think][planing]To create a travel plan that aligns with the user's preferences which has a high score, the key objectives are to select destinations known for live music, diverse takeout options (Korean, kosher, Japanese, seafood, and vegan). The budget constraint of $30 will also guide the choices.I should search for these requests,to see if there are places that meets the requirements.If I get the location correctly,I will give a proposal.If there is many choice,I will consider all proposals and give one proposal that is best. 

//HERE IS YOUR OUTPUT
You: [think][reasoning]I will search for cities or neighborhoods that are known for their vibrant music scenes and diverse food options, and then narrow it down to those that fit within the budget. I will consider multiple options and propose the best itinerary based on the gathered information.

"""
\end{lstlisting}

==> Prompt/navigation-planning/reflection.tex <==

\begin{lstlisting}[language=Python]
rompt_system_reflection="""
You are a travel agent. Book a set of three destinations that make the user most happy. Your objective is to maximize the "Final Score" at the end of the chat, which scores how well the final itinerary you proposed matches the user's preferences.

You and the user are limited to a fixed number of words in the chat. When the word count is below 0 then you will be forced to make your final proposal, which will be scored. You can also make proposals before the word count is up.

Please reflect on the  outcomes and consider the following points:
1. Identify why the current result is unsatisfactory.
2. Evaluate the effectiveness of past actions and thoughts. Propose improvements for the next steps. 
Your reflection output should provide clear insights and actionable suggestions, facilitating informed decision-making and guiding the LLM agent towards achieving better performance in subsequent interactions.
Ideally, it should contain flaw and improvements
Your response should use the following format:
[reflection]Reflection


Here is an example:
Your:[reflection] The flaw in the approach was not considering the user's budget constraint of $80 while proposing places like The Cakery, which exceeds this limit. Additionally, the proposal did not fully align with the user's updated preference for exclusively takeout options. The improvement would be to search for more budget-friendly takeout options that also allow reservations and offer panoramic views, ensuring all selections strictly adhere to the user's specified budget and preferences. 


"""
\end{lstlisting}

==> Table/MathSolver/knowledge_point_math.tex <==
\begin{table*}[htbp]
  \caption{Classification and Examples of Knowledge Points in Algebra/Geometry Data Sets}
  \label{tab:konwledge_point_math}
  \centering
  \resizebox{\textwidth}{!}{%
  \begin{tabular}{M{3cm}|M{5cm}|M{3cm}|M{5cm}}
    \toprule
    \multicolumn{2}{c|}{Algebra} & \multicolumn{2}{c}{Geometry} \\
    \multicolumn{1}{c|}{Knowledge Point}  & \multicolumn{1}{c|}{Example} & \multicolumn{1}{c|}{Knowledge Point} &  \multicolumn{1}{c|}{Example}  \\
    \midrule
    Complex Numbers  & Evaluate the sum $i^{100} + i^{101} + i^{102} + \cdots + i^{204}$. & Circles and Their Properties & A chord of length 8 cm is 6 cm away from the center of a circle. What is the radius of the circle?\\
    \midrule
    Algebra in Coordinate Geometry & A circle has a center at $(h, -1)$ and passes through the points $(0, 2)$ and $(4, 0)$. Find the radius of the circle. & Fundamentals of Trigonometry & The angle $\beta$ in a right triangle satisfies $\cos(\beta) = 12/13$. Find $\sin(2\beta)$. \\

    \midrule
    Exponents and Logarithms & If $3^{x}=4$, $4^{y}=5$, $5^{z}=6$, and $6^{w}=7$, find the value of $x \cdot y \cdot z \cdot w$. & Geometric Constructions and Coordinate Geometry & A rhombus $ABCD$ is situated in the coordinate plane with vertices $A(1, 2)$, $B(4, 6)$, and $C(7, 2)$. Determine the side length of the rhombus. \\
    
    \midrule
    Function Composition and Inverses & Let $f(x) = 2x + 3$. You are given that $g(f(x)) = 3x - 4$ for all $x$. Determine the value of $g(7)$. & Geometric Inequalities and Optimization Problems & Given a trapezoid with bases 10 units and 6 units, and one non-parallel side 4 units, find the maximum area of the trapezoid. \\
    \midrule
    Inequalities and Absolute Values & Find the product of integer solutions for $z$(-5 < z < 5) such that $|z^2 - 9|$ equals a prime number. & Polygons and Their Properties & Calculate the area of a regular dodecagon (12-sided polygon) with a circumradius (radius of the circumscribed circle) of 8 cm. \\
    
    \midrule
    Polynomials and Polynomial Operations & Give the factorization result of expression $(x + \sqrt{3})^3 + (y - \sqrt{3})^3$ & Properties of Right Triangles & In triangle $DEF$, $DE = EF = 13$ and $DF = 10$. Let $G$ be the foot of the altitude from $D$ to $\overline{EF}$. Compute the area of triangle $DGF$. \\
    
    \midrule
    Quadratic Equations and Functions & Determine the sum of all integer values of $b$ for which the quadratic equation $x^2 + bx + b = 0$ has integer solutions. & Quadrilateral Features and Classifications & Quadrilateral $ABCD$ has $AB = 4$, $BC = 5$, $CD = 6$, $DA = 7$, and diagonal $AC = 8$. Find the area of $ABCD$. \\
    
    \midrule
    Rational Functions and Expressions & Determine the domain of the function $$g(x) = \frac{3x-7}{x^2 - 4x + 3}.$$ Express your domain in interval notation. & Similar Triangles and Proportions & In triangle $DEF$, point $G$ divides side $DF$ in the ratio $2:3$. If the area of triangle $DEG$ is 12, find the area of triangle $EFG$.\\
    
    \midrule
    Sequences and Series & Consider the sequence defined recursively by $a_1 = 1000$ and $a_{n+1} = a_n - n$ for $n \geq 1$. Determine the smallest positive integer $n$ for which $a_n < 0$. & Three-Dimensional Geometry & A sphere with radius 7 is inscribed in a right circular cone. The cone's height is 24. Find the radius of the cone at its base. \\

    \midrule
    Systems of Linear Equations & Assume $x$ and $y$ satisfy the system of equations: $3x^2 + 4y = 16$ and $2x - y = 3$. Compute sum of possible value of $4x + 3y$. & Transformative Geometry and Symmetry & A circle with radius 5 cm is rotated about its center by 180 degrees. What is the total area covered by the circle during the rotation? \\
    \bottomrule
  \end{tabular}%
  }
\end{table*}

==> Table/MathSolver/praf_formal.tex <==
\begin{table*}[t]
  \caption{Experiment Results on Automatic Theorem Proving Tasks with $\Delta$ Accuracy}
  \label{tab:praf_formal}
  \centering
  \resizebox{\textwidth}{!}{%
  \begin{tabular}{c|ccccc|c|ccccc|c|ccccc|c}
    \toprule
    & \multicolumn{6}{c|}{Coq} & \multicolumn{6}{c|}{Lean 4} & \multicolumn{6}{c}{Isabelle} \\
    LLM & Pt & Rt & At & Ft & Acc(\%) & $\Delta$ Acc(\%) & Pt & Rt & At & Ft & Acc(\%) & $\Delta$ Acc(\%) & Pt & Rt & At & Ft & Acc(\%) & $\Delta$ Acc(\%) \\
    \midrule
    \texttt{llama3-8B} & / & / & / & / & 6.4 & / & / & / & / & / & 2.7 & / & / & / & / & / & 7.2 & / \\
    % \texttt{Claude-3.5} & -0.011 & \textbf{0.054} & \textbf{0.775} & 0.011 & \textbf{96.4} & +90.0 & 0.007 & \textbf{0.059} & \textbf{0.667} & \textbf{0.106} & \textbf{84.7} & +82.0 & 0.024 & 0.046 & \underline{0.512} & \textbf{0.076} & \textbf{74.8} & +67.6 \\
    % \texttt{gpt-4-turbo} & \textbf{0.035} & 0.044 & \underline{0.713} & \textbf{0.033} & \underline{86.5} & +80.1 & -0.027 & -0.009 & 0.365 & 0.020 & 41.4 & +38.7 & 0.034 & \textbf{0.047} & \textbf{0.536} & 0.014 & \underline{69.4} & +62.2 \\
    % \texttt{qwen2.5-32B} & 0.008 & 0.024 & 0.611 & 0.021 & 74.8 & +68.4 & -0.012 & \underline{0.012} & \underline{0.474} & \underline{0.044} & \underline{57.7} & +55.0 & \underline{0.050} & \textbf{0.047} & 0.439 & \underline{0.036} & 63.1 & +55.9 \\
    % \texttt{gpt-4o-mini} & \underline{0.028} & -0.026 & 0.388 & 0.017 & 49.6 & +43.2 & 0.003 & -0.010 & 0.404 & 0.024 & 39.6 & +36.9 & 0.027 & -0.009 & 0.243 & 0.018 & 36.0 & +28.8 \\
    % \texttt{doubao-pro-4k} & 0.002 & 0.040 & 0.203 & 0.000 & 31.5 & +25.1 & \textbf{0.024} & -0.006 & 0.042 & -0.019 & 16.2 & +13.5 & 0.039 & 0.012 & -0.060 & 0.010 & 5.4 & -1.8 \\
    % \texttt{GLM-4-air} & 0.013 & 0.016 & 0.115 & \underline{0.031} & 24.3 & +17.9 & -0.006 & 0.001 & 0.193 & 0.015 & 23.4 & +20.7 & 0.005 & -0.002 & 0.178 & 0.014 & 25.2 & +18.0 \\
    % \texttt{llama3-70B} & 0.011 & -0.147 & 0.185 & 0.002 & 14.4 & +8.0 & 0.000 & 0.002 & 0.038 & 0.025 & 7.2 & +4.5 & 0.035 & -0.037 & 0.152 & 0.003 & 24.3 & +17.1 \\
    % \texttt{Mistral-8X7B} & 0.010 & \underline{0.051} & 0.118 & 0.006 & 27.0 & +20.6 & -0.000 & -0.016 & 0.061 & -0.018 & 6.3 & +3.6 & \textbf{0.060} & 0.021 & -0.064 & -0.024 & 4.5 & -2.7 \\
    % \texttt{Mistral-7B} & 0.011 & 0.007 & 0.011 & -0.020 & 10.8 & +4.4 & \underline{0.011} & 0.005 & 0.005 & 0.007 & 8.1 & +5.4 & -0.007 & 0.009 & -0.070 & 0.005 & 0.0 & -7.2 \\
    \texttt{Claude-3.5} & 0.010 & \textbf{0.067} & \textbf{0.795} & \underline{0.027} & \textbf{96.4} & 90.0& 0.002 & \textbf{0.059} & \textbf{0.662} & \textbf{0.098} & \textbf{84.7} & 82.0& 0.025 & \underline{0.046} & \underline{0.523} & \textbf{0.082} & \textbf{74.8} & 67.6\\
    \texttt{gpt-4-turbo} & \underline{0.032} & 0.038 & \underline{0.706} & 0.024 & \underline{86.5} & 80.1& -0.015 & -0.006 & 0.375 & 0.033 & 41.4 & 38.7& 0.020 & \textbf{0.048} & \textbf{0.542} & 0.012 & \underline{69.4} & 62.2\\
    \texttt{qwen2.5-32B} & 0.014 & 0.029 & 0.615 & 0.026 & 74.8 & 68.4& -0.007 & 0.020 & \underline{0.486} & \underline{0.050} & \underline{57.7} & 55.0& \underline{0.048} & 0.041 & 0.434 & \underline{0.036} & 63.1 & 55.9\\
    \texttt{gpt-4o-mini} & \textbf{0.038} & -0.016 & 0.391 & 0.018 & 49.5 & 43.1& -0.013 & -0.020 & 0.396 & 0.007 & 39.6 & 36.9& 0.030 & -0.012 & 0.249 & 0.021 & 36.0 & 28.8\\
    \texttt{doubao-pro-4k} & 0.007 & 0.039 & 0.204 & 0.001 & 31.5 & 25.1& -0.017 & \underline{0.029} & 0.095 & 0.028 & 16.2 & 13.5& 0.035 & 0.007 & -0.064 & 0.004 & 5.4 & -1.8\\
    \texttt{GLM-4-air} & 0.015 & 0.016 & 0.115 & \textbf{0.033} & 24.3 & 17.9& -0.004 & 0.005 & 0.193 & 0.013 & 23.4 & 20.7& -0.006 & -0.006 & 0.176 & 0.017 & 25.2 & 18.0\\
    \texttt{llama3-70B} & 0.018 & -0.137 & 0.190 & 0.009 & 14.4 & 8.0& -0.005 & -0.000 & 0.030 & 0.020 & 7.2 & 4.5& 0.043 & -0.032 & 0.155 & 0.005 & 24.3 & 17.1\\
    \texttt{Mistral-8X7B} & 0.014 & \underline{0.056} & 0.122 & 0.014 & 27.0 & 20.6& \underline{0.003} & -0.017 & 0.068 & -0.018 & 6.3 & 3.6& \textbf{0.058} & 0.014 & -0.071 & -0.028 & 4.5 & -2.7\\
    \texttt{Mistral-7B} & 0.018 & 0.013 & 0.028 & -0.015 & 10.8 & 4.4& \textbf{0.020} & 0.011 & 0.012 & 0.012 & 8.1 & 5.4& -0.014 & 0.006 & -0.068 & 0.003 & 0.0 & -7.2\\
    \midrule
    \texttt{best} & / & / & / & / & \textit{94.6} & \textit{+88.2} & / & / & / & / & \textbf{\textit{87.4}} & \textit{+84.7} & / & / & / & / & \textbf{\textit{78.4}} & \textit{+71.2} \\
    \bottomrule
  \end{tabular}}
\end{table*}

==> Table/MathSolver/praf_math.tex <==
\begin{table*}[t]
  \caption{PRAF Experiment Results on Mathematics Tasks with $\Delta$ Accuracy}
  \label{tab:praf_math}
  \centering
  \resizebox{\textwidth}{!}{%
  \begin{tabular}{c|ccccc|c|ccccc|c}
    \toprule
    & \multicolumn{6}{c|}{Algebra} & \multicolumn{6}{c}{Geometry} \\
    LLM & Pt & Rt & At & Ft & Acc(\%) & $\Delta$ Acc(\%) & Pt & Rt & At & Ft & Acc(\%) & $\Delta$ Acc(\%) \\
    \midrule
    \texttt{llama3-8B-instruct} & / & / & / & / & 21.6 & / & / & / & / & / & 14.4 & / \\
    % \texttt{Claude-3.5-Sonnet} & 0.029 & \textbf{0.176} & 0.397 & \underline{0.031} & \underline{84.4} & +62.8 & 0.056 & \textbf{0.077} & 0.471 & \underline{0.039} & \underline{82.4} & +68.0 \\
    % \texttt{gpt-4-turbo} & 0.060 & 0.084 & \textbf{0.456} & 0.020 & 83.2 & +61.6 & 0.034 & 0.040 & \underline{0.526} & 0.019 & 78.0 & +63.6 \\
    % \texttt{qwen2.5-32B} & 0.067 & \underline{0.150} & \underline{0.444} & 0.015 & \textbf{86.8} & +65.2 & 0.074 & \underline{0.064} & \textbf{0.530} & \textbf{0.044} & \textbf{86.4} & +72.0 \\
    % \texttt{gpt-4o-mini} & \underline{0.078} & 0.038 & 0.318 & \textbf{0.032} & 67.2 & +45.6 & \underline{0.076} & 0.041 & 0.395 & 0.027 & 63.6 & +49.2 \\
    % \texttt{doubao-pro-4k} & \textbf{0.130} & 0.094 & 0.182 & 0.005 & 60.8 & +39.2 & \textbf{0.108} & 0.041 & 0.184 & -0.006 & 46.0 & +31.6 \\
    % \texttt{GLM-4-air} & 0.052 & 0.065 & 0.343 & -0.004 & 68.8 & +47.2 & 0.054 & 0.018 & 0.346 & 0.006 & 57.6 & +43.2 \\
    % \texttt{llama3-70B} & 0.035 & 0.047 & 0.317 & 0.006 & 63.6 & +42.0 & 0.019 & 0.012 & 0.335 & 0.006 & 50.8 & +36.4 \\
    % \texttt{Mistral-8X7B} & 0.009 & -0.010 & 0.190 & -0.008 & 39.2 & +17.6 & 0.006 & 0.018 & 0.142 & -0.022 & 28.4 & +14.0 \\
    % \texttt{Mistral-7B} & -0.065 & -0.014 & -0.051 & -0.005 & 8.0 & -13.6 & -0.060 & 0.011 & -0.038 & -0.007 & 6.4 & -8.0 \\
    \texttt{Claude-3.5-Sonnet} & 0.021 & \textbf{0.177} & 0.398 & \underline{0.031} & \underline{84.4} & 62.8& 0.055 & \textbf{0.085} & 0.486 & \textbf{0.054} & \underline{82.4} & 68.0\\
    \texttt{gpt-4-turbo} & 0.058 & 0.082 & \textbf{0.456} & 0.020 & 83.2 & 61.6& 0.038 & 0.047 & \underline{0.527} & 0.025 & 78.0 & 63.6\\
    \texttt{qwen2.5-32B} & 0.059 & \underline{0.146} & \underline{0.436} & 0.011 & \textbf{86.8} & 65.2& \underline{0.071} & \underline{0.067} & \textbf{0.530} & \underline{0.051} & \textbf{86.4} & 72.0\\
    \texttt{gpt-4o-mini} & \underline{0.070} & 0.020 & 0.313 & \textbf{0.053} & 67.2 & 45.6& 0.065 & 0.024 & 0.368 & 0.035 & 63.6 & 49.2\\
    \texttt{doubao-pro-4k} & \textbf{0.124} & 0.086 & 0.178 & 0.004 & 60.8 & 39.2& \textbf{0.105} & 0.032 & 0.186 & -0.007 & 46.0 & 31.6\\
    \texttt{GLM-4-air} & 0.053 & 0.069 & 0.346 & 0.004 & 68.8 & 47.2& 0.059 & 0.019 & 0.349 & 0.006 & 57.6 & 43.2\\
    \texttt{llama3-70B} & 0.040 & 0.051 & 0.321 & 0.007 & 63.6 & 42.0& 0.015 & 0.011 & 0.333 & 0.005 & 50.8 & 36.4\\
    \texttt{Mistral-8X7B} & 0.006 & -0.010 & 0.190 & -0.010 & 39.2 & 17.6& 0.004 & 0.016 & 0.138 & -0.018 & 28.4 & 14.0\\
    \texttt{Mistral-7B} & -0.065 & -0.015 & -0.053 & -0.003 & 8.0 & -13.6& -0.055 & 0.014 & -0.035 & -0.004 & 6.4 & -8.0\\
    \bottomrule
  \end{tabular}%
  }
\end{table*}

==> Table/OS/OS_classification.tex <==
\begin{table*}[htbp]
  \caption{Categories and Examples of Operating System Datasets}
  \label{tab:konwledge_point_os}
  \centering
  \resizebox{\textwidth}{!}{%
  \begin{tabular}{M{3cm}|M{5cm}|M{3cm}|M{5cm}}
    \toprule
    \multicolumn{1}{c|}{Category}  & \multicolumn{1}{c|}{Category Description} & \multicolumn{1}{c|}{Related Commands} &  \multicolumn{1}{c|}{Example Task Description}  \\
    \midrule
    File System Manipulation  
    & Evaluate the knowledge of basic file system manipulation operation such as creating, deleting, copying, moving, compressing and listing files and directories.
    & mkdir, touch, zip, tar, ls, rm
    & List all files larger than 1MB inside the '/var/log' directory and write the list to a file named 'large\_files.txt' in the home directory.\\
    
    \midrule
    System Setting 
    & Evaluate the knowledge of system setting such as disk partition, OS version, user management.
    & df, useradd, groupadd, uname, chmod, whoami, chown
    & A user needs permission to read a file in '/var/private/info.txt'. Grant read access to all users. \\

    \midrule
    Process Running 
    & Evaluate the knowledge of processes management
    & renice, gcc, g++, python
    & Change the priority of the process with PID stored in /tmp/pidfile to a nice value of 10. \\

    \bottomrule
  \end{tabular}%
  }
\end{table*}

==> Table/RoCo/praf_GPT.tex <==
\begin{table*}[h]
  \caption{Experimental Results on Robot Cooperation(100 tasks)}
  \label{tab:praf_RoCo}
  \centering
  \resizebox{\textwidth}{!}{%
  \begin{tabular}{ccccccc}
    \toprule
    LLM & Pt & Rt & At & Ft & Reward (\%) & $\Delta$ Reward (\%) \\
    \midrule
    \texttt{Llama3-8B-instruct(Default)} 
    & - & - & - & - & 8.85 & - \\
    \texttt{claude-3.5-sonnet} & 0.0888 & \textbf{0.4031} & \textbf{0.349} & 0.0054 & \textbf{92.63} & \underline{84.64999999999999}\\
    \texttt{gpt-4o-mini} & 0.0971 & 0.1545 & 0.2181 & 0.0047 & 55.43 & 47.45\\
    \texttt{glm-4-airx} & 0.0067 & 0.0837 & 0.0182 & -0.0141 & 17.43 & \textbf{9.45}\\
    \texttt{gpt-4-turbo-0409} & 0.0821 & \underline{0.3447} & \underline{0.3216} & \underline{0.0137} & \underline{84.17999999999999} & 76.19999999999999\\
    \texttt{qwen2.5-32b-ins} & \textbf{0.1088} & 0.211 & 0.3167 & 0.0097 & 72.59 & 64.61\\
    \texttt{Mistral-7B-Instruct} & 0.009 & -0.019 & -0.0191 & 0.0009 & 5.17 & -2.8099999999999996\\
    \texttt{Llama-3-70B-Instruct} & 0.0637 & 0.1259 & 0.1766 & 0.0045 & 45.06 & 37.080000000000005\\
    \texttt{doubao-pro-4k} & \underline{0.0989} & 0.0896 & 0.0009 & \textbf{0.0313} & 30.049999999999997 & 22.069999999999997\\
    \texttt{Mistral-8X7B-instruct} & 0.0022 & 0.0168 & 0.066 & 0.0038 & 16.869999999999997 & 8.889999999999997\\
    \midrule
    \texttt{best} & / & / & / & / & \textit{92.63} & \textit{+83.68}\\
    \bottomrule
  \end{tabular}}
\end{table*}

==> Table/RoCo/praf_Llama_3_8b.tex <==
\begin{table*}[h]
  \caption{Experimental Results on Robot Cooperation(100 tasks)}
  \label{tab:praf_RoCo}
  \centering
  \resizebox{\textwidth}{!}{%
  \begin{tabular}{ccccccc}
    \toprule
    LLM & Pt & Rt & At & Ft & Reward (\%) & $\Delta$ Reward (\%) \\
    \midrule
    \texttt{Llama3-8B-instruct(Default)} 
    & - & - & - & - & 8.85 & - \\
    \texttt{claude-3.5-sonnet} & \textbf{0.1140} & \textbf{0.3879} & \textbf{0.3186} & \textbf{0.0172} & \textbf{92.63} & \textbf{+83.78}\\
\texttt{gpt-4o-mini} & 0.0748 & 0.1888 & 0.1957 & -0.0034 & 54.43 & +45.58\\
\texttt{glm-4-airx} & -0.0235 & 0.1157 & 0.0078 & -0.0124 & 17.60 & +8.75\\
\texttt{gpt-4-turbo-0409} & \underline{0.1069} & \underline{0.3292} & \underline{0.3162} & 0.0011 & \underline{84.18} & \underline{+75.33}\\
\texttt{qwen2.5-32b-ins} & 0.0895 & 0.2683 & 0.2768 & 0.0029 & 72.59 & +63.74\\
\texttt{Mistral-7B-Instruct} & -0.0142 & -0.0001 & -0.0211 & -0.0014 & 5.17 & -3.68\\
\texttt{Llama-3-70B-Instruct} & 0.0426 & 0.1524 & 0.1750 & -0.0078 & 45.06 & +36.21\\
\texttt{doubao-pro-4k} & 0.0208 & -0.004 & 0.2043 & -0.0122 & 29.75 & +20.90\\
\texttt{Mistral-8X7B-instruct} & -0.0049 & 0.0329 & 0.0521 & \underline{0.0040} & 17.27 & +8.42\\
    \midrule
    \texttt{best} & / & / & / & / & \textit{92.63} & \textit{+83.78}\\
    \bottomrule
  \end{tabular}}
\end{table*}
